How Generative Adversarial Networks and Their Variants Work: An Overview

Generative Adversarial Networks (GAN) have received wide attention in the machine learning field for their potential to learn high-dimensional, complex real data distribution. Specifically, they do not rely on any assumptions about the distribution and can generate real-like samples from latent space in a simple manner. This powerful property leads GAN to be applied to various applications such as image synthesis, image attribute editing, image translation, domain adaptation and other academic fields. In this paper, we aim to discuss the details of GAN for those readers who are familiar with, but do not comprehend GAN deeply or who wish to view GAN from various perspectives. In addition, we explain how GAN operates and the fundamental meaning of various objective functions that have been suggested recently. We then focus on how the GAN can be combined with an autoencoder framework. Finally, we enumerate the GAN variants that are applied to various tasks and other fields for those who are interested in exploiting GAN for their research.

==> latent_space/ppgn.tex <==
\subsubsection{Sampling from latent space} \label{ppgn}
Plug and Play Generative Networks (PPGN) \cite{PPGN} is a type of a generative model derived from sampling techniques. It consists of a generator network $G$ and a condition network $C$, where $G$ produces data, and $C$ performs conditioning through an image classifying function. More specifically, the PPGN framework is derived from activation maximization. Using a chain rule, a joint probability can be split into a constraint that allows data to be in class $y$ and a constraint that allows data to be on the manifold of the image distribution to sample the data as follows:
\begin{align}
p(x,y) = p(x)p(y|x) 
\end{align}
In fact, it is common to generate data with a class given as $y= y_c$. This task can be interpreted as a problem to sample data from conditional distribution $p(x|y=y_c)$ and this can be represented by Bayes' rule as follows:
\begin{align}
p(x|y=y_c) \propto p(x)p(y=y_c|x)
\end{align}
Maximizing $p(x|y=y_c)$ by the activation maximization method is equivalent to maximizing the likelihood that $x$ remains in the manifold of the image distribution and likelihood that the generated data is in the $y_c$ class. $G$ and $C$ perform two tasks respectively. To maximize these likelihoods, we need samples from the data distribution.
%PPGN \cite{PPGN} introduces the MALA-approx sampler to sample the data maximizing likelihood of $p(x)$. To derive this, \cite{PPGN} introduces various existing samplers. Metropolis-Hastings (MH) sampler has a disadvantage of slow mixing and computing $p(x)$ to calculate acceptance ratio.

%For fast mixing, Metropolis-adjusted Langevin algorithm (MALA) sampler was proposed. Unlike MH sampler, $x_t + 1$ is selected in direction of increasing log-likelihood through the gradient ascent rather than in direction of random noise, so MALA sampler mixes fast. However, there is still a problem that $p(x)$ must be computed when calculating the acceptance ratio, which is the second problem of the MH algorithm.
%On the other hand, the SGLD method is a sampling method that can form a probability proposal with only a subset of data. This is possible by using SGD with noise, skipping the accept-reject step and decaying the step size. 
%The proposed method is based on SGLD, decaying the step size and eliminating the accept-reject step. The SGD, whose step size gradually decreases, produces unbiased samples asymptotically and has the effect of noise. If the step size is 0 instead the acceptance ratio is 1, the sampler produces reasonable samples. The MALA-approx sampler can be formulated as follows.
%\begin{align}
%x_{t+1}=x_t + \frac{\sigma^2}{2}\nabla \log p(x_t) + N(0,\sigma^2)
%\end{align}
%$\nabla \log p(x_t)$ can be separated by $\partial \log p(x_t)/\partial x_t$ and $\partial \log p(y=y_c|x_t)/\partial x_t$ using (19), where the former is the direction to increase the likelihood of data distribution and the latter is the direction in which the probability of $y = y_c$ given the current image $x_t$ is higher. You can change the sampling aspect by adjusting the weighting factors for these two terms. The former can be approximated with the reconstruction error of pretrained Denoising Autoencoder (DAE). This enables sampling without directly computing $p(x)$. Also, the latter can be computed from the classifier, so the whole process is called PPGN-$x$.

% DAE 가 먼지 설명 필요. PPGN-x 는 삭제
Data can be sampled directly from the sampler, but sampling in a high-dimensional space such as image data suffers from poor mixing \cite{mala}. Therefore, PPGN introduces latent variable $z_t$ in a low-dimensional latent space. It samples $z_t$ and $z_t$ is used as the input of the generator to extract data. The generator is trained by the feature matching loss proposed in \citet{Improved}, which is the $l_2$ loss between the real data and the generated data in the feature space. The next sample $z_{t + 1}$ is selected which increases the class probability by the gradient back-propagated from the classifier output as follows: 
\begin{align}
z_{t+1}=z_t + \epsilon_1 (R_z(z_t)-z_t) + \epsilon_2 \frac{\partial\log C_c(G(z_t))}{\partial G(z_t)} \frac{\partial G(z_t)}{\partial z_t},
\end{align}
where $ R_h(\cdot) $ is the reconstruction function of the denoising auto-encoder (DAE) \cite{dae} in the latent space. DAE is an unsupervised learning algorithm that extracts robust features by reconstructing original data from noisy data. $C_c(\cdot)$ denotes the output unit of classifier corresponding to class $y_c$.
Sometimes, DAE does not model well owing to unconstrained density estimation. Joint PPGN learns that latent variables become generated data and then decodes such generated data back to latent variables. In this manner, Joint PPGN can sample a latent variable $h$ which is more constrained for $x$. It learns the DAEs for $h_t$, $z_t$ (with the noise vector $\eta$), and $x_t$ that share parameters as seen in Figure~\ref{fig:jointppgnz}. Actually, encoders are frozen and only the generator is learned. Its loss function has four loss terms, an adversarial loss term, and the $l_2$ reconstruction loss terms for $h_t$, $z_t$, and $x_t$. 
%In this way, PPGN aims to generate high-resolution, high-quality images.
\begin{figure} [h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/ppgnz.pdf}
        \caption{PPGN-z}
        \label{fig:ppgnz}
    \end{subfigure} 
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{figures/jointppgnz.pdf}
        \caption{Joint PPGN-z}
        \label{fig:jointppgnz}
    \end{subfigure}
    \caption{PPGN \cite{PPGN}}\label{fig:PPGN}
\end{figure}
